New links between PDE's and Voronoi patterns

This paper presents a range of results in partial differential equations (PDEs) in which Voronoi patterns arise. We investigate the connection between the solution to an elliptic equation and its probabilistic interpretation as a stochastic colonization game. An agent-based model is designed and implemented to generate the Voronoi cells simulating experimental results with bacteria. We also consider the analytical solution to the problem, which enables us to define what we call a harmonic Voronoi tessellation. We analyze parabolic equations in Riemannian manifolds, which have important applications in chemical reactions and diffusive fronts. By utilizing short-time heat kernel estimates, we demonstrate that the interaction of $n$ point sources gives rise to a Voronoi tessellation. We recall some well-known results of wavefronts interactions from point light sources and the Huygens principle. We apply results about the particular set of weak solutions to the eikonal equation to characterize Voronoi patterns arising in this context as rectifiable sets. Finally, we present an optimal transport problem and the corresponding Monge-Amp\`ere equation, in which a uniform measure is transported to a sum of $n$ Dirac masses with a cost given by the Euclidean distance. These problems are naturally linked to power sets, a generalization of Voronoi tessellations.

==> algorithm.tex <==
\subsection{Agent based model that recovers Voronoi cells}


\subsection{Code}\label{sec:Code}

\begin{tiny}
\begin{lstlisting}
function VoronoiAgents()

% Simulation of Brownian motion of 'np' Particles for T seconds
clear;
clc;
T= input('Enter the Time Period: ');     % Time (in Seconds)
N=100*T;                              % Number of Impulses/change in track
h=1/10;
nS=input('Enter the Number of sources: ');    % Number of sources
np=100;                               %Number of particles per source

% Domain
xL=2;
yL=2; 

cmap = hsv(nS); % Creates a np-by-3 set of colors from the HSV colormap

% Initial position of the np sources
x=zeros(nS,np,N);
y=zeros(nS,np,N);
for i=1:nS
    x(i,:,1)=rand(1)*xL;
    y(i,:,1)=rand(1)*yL;
end

clf;
figure(1);
xlim([0,xL]);
ylim([0,yL]);

hold on;
% plot the sources
for k=1:nS
    theta = linspace(0,2*pi);
    xc = .2*cos(theta) + x(k,1,1);
    yc = .2*sin(theta) + y(k,1,1);
    plot(xc,yc,'Color',cmap(k,:));
end

%cont=1;
%part=zeros(np,1);
% Iteration to store positions of particles
for t=1:N  %time
	for j=1:np %number of particles per source
        for i=1:nS   %number of sources
            rx=randn(); ry=randn();
            if  (x(i,j,t)+h*rx>=xL || x(i,j,t)+h*rx<=0 
            || y(i,j,t)+h*ry>=yL ||  y(i,j,t)+h*ry<=0 )                     
                x(i,j,t+1)=x(i,j,1);        % retruns to its source
                y(i,j,t+1)= y(i,j,1);
                continue;                   % next iteration i
            else  % Valid position
                x(i,j,t+1)=x(i,j,t)+h*rx;          
                y(i,j,t+1)=y(i,j,t)+h*ry;         
                if (t>5)
                   c=coalition(x,y,i,j,t,nS,np);       
                   if c>0 % coalition            
                     x(i,j,t+1)=x(i,j,1); 
                     y(i,j,t+1)=y(i,j,1);  
                   end
               end
            end
        end
    end
end

% Plotting of the particles. 
for i=1:nS
    X=x(i,1:np,1:N);
    X=squeeze(X);
    Y=y(i,1:np,1:N);
    Y=squeeze(Y);
    for j=1:np
        plot(X(j,:),Y(j,:),'.','Color',cmap(i,:));
    end
end

% plot the sources
for k=1:nS
    theta = linspace(0,2*pi);
    xc = .2*cos(theta) + x(k,1,1);
    yc = .2*sin(theta) + y(k,1,1);
    plot(xc,yc,'k');
    %plot(xc,yc,'Color',cmap(k,:));
    %plot(x(k,1,1),y(k,1,1),'r*');
end
voronoi(x(:,1,1),y(:,1,1),'k');
end
                    
function c=coalition(x,y,S,p,t,nS,np)
epsilon=.01;
c=0;
D=zeros(1,t);
% S, p last particle that moved
for i=1:nS
    if i==S % same source
        continue
    end
    for j=1:np
    % Distance between last movement and the trajectory of the other 
    % particles from 1 to t
        for k=1:t
            D(k)=sqrt((x(S,p,t+1)-x(i,j,k))^2+(y(S,p,t+1)-y(i,j,k))^2);
        end
        [d,idx]=min(D);
        if d<epsilon
            %if min(pdist2([x(S,p,t+1),y(S,p,t+1)],[x(i,j,t),y(i,j,t)]))<epsilon
            c=[i,j,idx];   %coalition with particle j, source j time idx
            return  % return c
        end
    end
end
return %no coalition
end
\end{lstlisting}
\end{tiny}



